Sieve: Actionable Insights from Monitored Metrics in Microservices

Major cloud computing operators provide powerful monitoring tools to understand the current (and prior) state of the distributed systems deployed in their infrastructure. While such tools provide a detailed monitoring mechanism at scale, they also pose a significant challenge for the application developers/operators to transform the huge space of monitored metrics into useful insights. These insights are essential to build effective management tools for improving the efficiency, resiliency, and dependability of distributed systems. This paper reports on our experience with building and deploying Sieve - a platform to derive actionable insights from monitored metrics in distributed systems. Sieve builds on two core components: a metrics reduction framework, and a metrics dependency extractor. More specifically, Sieve first reduces the dimensionality of metrics by automatically filtering out unimportant metrics by observing their signal over time. Afterwards, Sieve infers metrics dependencies between distributed components of the system using a predictive-causality model by testing for Granger Causality. We implemented Sieve as a generic platform and deployed it for two microservices-based distributed systems: OpenStack and ShareLatex. Our experience shows that (1) Sieve can reduce the number of metrics by at least an order of magnitude (10 - 100$\times$), while preserving the statistical equivalence to the total number of monitored metrics; (2) Sieve can dramatically improve existing monitoring infrastructures by reducing the associated overheads over the entire system stack (CPU - 80%, storage - 90%, and network - 50%); (3) Lastly, Sieve can be effective to support a wide-range of workflows in distributed systems - we showcase two such workflows: orchestration of autoscaling, and Root Cause Analysis (RCA).

==> cluster-evaluation.tex <==
\subsubsection{Top clustering}

Service: spelling

Silhouette Coefficient: 0.940260

\begin{table*}[t]
\begin{tabular}{l | l | l | l}
  Cluster & Graphical Evaluation & Application Logic & Shape-based distance \\ \hline

  1   &
  Yes &
  Yes &
  Yes \\

  1   &
  Yes &
  Yes &
  Yes (usage percent is an outlier) \\
\end{tabular}
\end{table*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/spelling-cluster-4_2.pdf}
\caption{Service: spelling, Cluster: 1 of 2}
\label{fig:mutual-information-score-1}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/spelling-cluster-4_4.pdf}
\caption{Service: spelling, Cluster: 2 of 2}
\label{fig:mutual-information-score-2}
\end{figure*}

\subsubsection{Middle-quality clustering}

Service: real-time

Silhouette Coefficient: 0.597103

\begin{table*}[t]
\begin{tabular}{l | l | l | l}
  Cluster & Graphical Evaluation & Application Logic & Shape-based distance \\ \hline

  1   &
  Yes &
  Yes &
  Yes \\

  2   &
  Yes &
  Yes &
  Yes \\

  3   &
  No  &
  Yes &
  No \\

  4   &
  No  &
  Yes &
  No \\

  5   &
  Yes &
  No  &
  yes \\
\end{tabular}
\end{table*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/real-time-cluster-5_1.pdf}
\caption{Service: real-time, Cluster: 1 of 5}
\label{fig:mutual-information-score-3}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/real-time-cluster-5_2.pdf}
\caption{Service: real-time, Cluster: 2 of 5}
\label{fig:mutual-information-score-4}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/real-time-cluster-5_3.pdf}
\caption{Service: real-time, Cluster: 3 of 5}
\label{fig:mutual-information-score-5}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/real-time-cluster-5_4.pdf}
\caption{Service: real-time, Cluster: 4 of 5}
\label{fig:mutual-information-score-6}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/real-time-cluster-5_5.pdf}
\caption{Service: real-time, Cluster: 5 of 5}
\label{fig:mutual-information-score-7}
\end{figure*}

\subsubsection{Lowest quality clustering}

Service: web

Silhouette Coefficient: 0.390812

\begin{table*}[t]
\begin{tabular}{l | l | l | l}
  Cluster & Graphical Evaluation & Application Logic & Shape-based distance \\ \hline

  1   &
  No &
  No &
  No \\

  2   &
  No  &
  Yes &
  No  \\

  3   &
  Yes &
  Yes &
  Yes \\

  4   &
  Yes &
  Yes &
  No  \\

  5   &
  Yes &
  Yes &
  No  \\

  6   &
  Yes &
  Yes &
  Yes \\

  7   &
  No  &
  Yes &
  Yes \\
\end{tabular}
\end{table*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/web-cluster-7_1.pdf}
\caption{Service: web, Cluster: 1 of 7}
\label{fig:mutual-information-score-8}

\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/web-cluster-7_2.pdf}
\caption{Service: web, Cluster: 2 of 7}
\label{fig:mutual-information-score-9}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/web-cluster-7_3.pdf}
\caption{Service: web, Cluster: 3 of 7}
\label{fig:mutual-information-score-10}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/web-cluster-7_4.pdf}
\caption{Service: web, Cluster: 4 of 7}
\label{fig:mutual-information-score-11}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/web-cluster-7_5.pdf}
\caption{Service: web, Cluster: 5 of 7}
\label{fig:mutual-information-score-12}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/web-cluster-7_6.pdf}
\caption{Service: web, Cluster: 6 of 7}
\label{fig:mutual-information-score-13}
\end{figure*}

\begin{figure*}[t]
\includegraphics[scale=.6]{figures/clusters/web-cluster-7_7.pdf}
\caption{Service: web, Cluster: 7 of 7}
\label{fig:mutual-information-score-14}
\end{figure*}


==> implementation-general.tex <==
\section{\sys Implementation}
\label{sec:implementation-general}

- [ ] Related Work: Autoscaling
  - [ ] half page
- [ ] Conclusion
  - [ ] Summarize problem statement
  - [ ] How it was solved

\paragraph{Our Approach: sysdig}
A new project called sysdig~\cite{sysdig} introduces a new more efficient way to
observe system calls. It provides a new kernel module which provides system
calls with included application context as an event stream to an userspace
application. It provides a sophisticated filter language and allows to
post-process with custom Scripts written in the Lua programming language.
Because of the application context provided, network calls made by a process can
be mapped onto the corresponding service. Here sysdig can also provide
information of the application container in which the process is running, as
well as which peer is the initiator of the connection and which peer provides
the service. To use sysdig in a distributed setting an application was written
to start sysdig on multiple hosts at once and collect the results.

This tool only imposes little overhead and can be also run in production environment on a
subset of machines which contains at least one instance for each component (TODO:
figure depicting multiple machines and sysdig, microbenchmark regarding
overhead?).

\section{auto-scaling specific implementation}
this part should be part of the auto-scaling implementation because it describes the
load generator for sharelatex.

for the root-cause analysis, the load generation is handled by an existing tool called
Rally.

\iea{You can refer to TPC-W, in which the user was taking an action according
to some probabilities. There can also be other load generators that behave the
same way; maybe RUBIS? - TPC-W uses negative expontial distribution. It does
not simulate users and only distinguish between read/write. For evaluation
I would take the 2 workloads from NASA + WorldCup (real-workloads)}
For our application a loadgenerator was written, which simulates users. Each
user has list of potential action it can draw from at random. Actions here can
have different weight. Like a real user they follow the same path through the
website. Each action triggers requests a real browser would trigger, if a
certain button is clicked or a page is visited. Between each action the virtual
user waits for a number of time. This time is normal distributed, which is
required for later analytics~\ref{ssec:granger-causality}.

\iea{Where did the `stationary' come from? Why is it required? Is this used for
granger causality? clustering? Without knowing why we make it `stationary',
it's confusing.}

In addition to the thinking time of users also the arrival and departure process
of users have to follow normal distribution. One prerequisite for normal
distribution is that load caused by arriving/departing users is stationary. This
means that the probability of the current load does not depend on the past load.
The naïve way would be to add or remove a random number of users at some point
in time. However this load distribution would follow a random walk model as the
number of users depend on the previous number of users. Instead a new random
number of users is generated each time using a normal distributed random
generator.

\textbf{obtaining metrics} In our case Linux's Cgroups~\cite{cgroups} were used due
components were deployed as containers. In this case system resource usage of
different components can be distinguished.


==> space-tricks.tex <==
% -*- root: main.tex -*-

%space left between floats.
\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}
% space above caption
\setlength{\abovecaptionskip}{2mm}
%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{1}

%\usepackage[small,compact,noindentafter]{titlesec}
%\usepackage[compact]{titlesec}

%\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
%\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
%\titlespacing{\section}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}

\usepackage[inline]{enumitem}
\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

\usepackage[subtle]{savetrees}
% \usepackage[moderate]{savetrees}


==> tables/tab-influxdb-overhead.tex <==
\begin{tabular}{llll}
\toprule
Metric &      Before &       After & Size [\%] \\
\midrule
CPU time [s]          &      0.45 G&    0.085 G  &              18.8  \\
DB size [KB]          &      588.8 &       36.0  &               6.1  \\
Incoming traffic [MB] &       11.1 &        2.3  &              20.6  \\
Outgoing traffic [KB] &       15.1 &        7.4  &              49.3  \\
\bottomrule
\end{tabular}

